Nearest Neighbour Few-Shot Learning for Cross-lingual Classification

Even though large pre-trained multilingual models (e.g. mBERT, XLM-R) have led to significant performance gains on a wide range of cross-lingual NLP tasks, success on many downstream tasks still relies on the availability of sufficient annotated data. Traditional fine-tuning of pre-trained models using only a few target samples can cause over-fitting. This can be quite limiting as most languages in the world are under-resourced. In this work, we investigate cross-lingual adaptation using a simple nearest neighbor few-shot (<15 samples) inference technique for classification tasks. We experiment using a total of 16 distinct languages across two NLP tasks- XNLI and PAWS-X. Our approach consistently improves traditional fine-tuning using only a handful of labeled samples in target locales. We also demonstrate its generalization capability across tasks.

==> paper.tex <==
% https://arxiv.org/pdf/2005.00633.pdf
% https://arxiv.org/pdf/2003.02739.pdf
% https://arxiv.org/pdf/2006.15486.pdf
% https://arxiv.org/pdf/2004.13889.pdf
% https://arxiv.org/pdf/1904.09077.pdf


% naive
% https://maelfabien.github.io/machinelearning/NLP_5/#

% Exploiting Cloze Questions for Few Shot Text Classification and Natural Language Inference
% https://arxiv.org/pdf/2001.07676.pdf

% When Low Resource NLP Meets Unsupervised Language Model: Meta-pretraining Then Meta-learning for Few-shot Text Classification
% https://arxiv.org/pdf/1908.08788.pdf


% Improving Few-shot Text Classification via Pretrained Language Representations
% https://arxiv.org/pdf/1908.08788v1.pdf

% https://github.com/zxlzr/FewShotNLP
